Tweezers: A Framework for Security Event Detection via Event Attribution-centric Tweet Embedding

Twitter is recognized as a crucial platform for the dissemination and gathering of Cyber Threat Intelligence (CTI). Its capability to provide real-time, actionable intelligence makes it an indispensable tool for detecting security events, helping security professionals cope with ever-growing threats. However, the large volume of tweets and inherent noises of human-crafted tweets pose significant challenges in accurately identifying security events. While many studies tried to filter out event-related tweets based on keywords, they are not effective due to their limitation in understanding the semantics of tweets. Another challenge in security event detection from Twitter is the comprehensive coverage of security events. Previous studies emphasized the importance of early detection of security events, but they overlooked the importance of event coverage. To cope with these challenges, in our study, we introduce a novel event attribution-centric tweet embedding method to enable the high precision and coverage of events. Our experiment result shows that the proposed method outperforms existing text and graph-based tweet embedding methods in identifying security events. Leveraging this novel embedding approach, we have developed and implemented a framework, Tweezers, that is applicable to security event detection from Twitter for CTI gathering. This framework has demonstrated its effectiveness, detecting twice as many events compared to established baselines. Additionally, we have showcased two applications, built on Tweezers for the integration and inspection of security events, i.e., security event trend analysis and informative security user identification.

==> tables/additional_criteria.tex <==
\begin{table*}[h]
\diffnote{RC1}
\ra{1.5}
\begin{mdframed}[backgroundcolor=brown!10]
\caption{Detailed Criteria for Annotating Tweets}
\adjustbox{width=.8\textwidth, center}{
\begin{tabular}{ll}
\toprule
\textbf{Type} & \textbf{Annotation Guidelines} \\ 
\midrule
\textbf{General Analysis} & Tweets are analyzed and classified based on the contained cybersecurity content. \\
\textbf{Uninformative}  & Tweets lacking clarity or detailed information for classification are marked Uninformative. \\
\textbf{Security-Related Hiring} & Tweets regarding job postings in security fields are annotated as Non-security. \\
\textbf{CVE Mentions} & Classified by detailed explanation present, otherwise annotated under Vulnerability. \\
\textbf{Mentions of Hacking Groups} & Classified based on known activities of the group; otherwise, marked Uninformative. \\
\textbf{Fraud Types} & Election fraud is annotated as non-security; other frauds as Fraud/Phishing. \\
\textbf{Security Keyword Enumeration} & Tweets listing security keywords without context are considered Uninformative. \\
\textbf{Fundraising for Security Firms} & Tweets about fundraising activities for security firms are annotated as Non-security. \\
\bottomrule
\end{tabular}}
\label{tab:additional_criteria}
\end{mdframed}
\end{table*}


==> tables/baseline_comparison.tex <==
\begin{table*}[ht!]
    \centering
    \caption{Comparison of \model{} with prior work.}
    \ra{1.2}
    \begin{adjustbox}{width=.95\linewidth, center}
	\begin{tabular}{lc|ccc}
	\toprule
    & \makecell[c]{Fine-grained Event \\ Detection} & \makecell[c]{Filtering Method \\ (\textit{Limitation 1})} & \makecell[c]{Clustering Input Features \\ (\textit{Limitation 2})} & \makecell[c]{Multi-label \\ (\textit{Limitation 3})}  \\
    \midrule
    \makecell[l]{Yagcioglu et al.~\cite{CYDEC}, Sabottke et al.~\cite{sabottke2015vulnerability},\\ 
    Ritter et al.~\cite{ritter2015weakly}, Zong et al.~\cite{TwitterThreats}, Le et al.~\cite{noveltyCVE}} & \xmarknew & N/A & N/A & \xmarknew \\
    \midrule
    Bose et al.~\cite{bose} & \cmarknew & Manual annotation & Text (TF-IDF) & \xmarknew\\
    SONAR~\cite{le2017sonar} & \cmarknew & Keyword-based & Text (GloVe) & \xmarknew\\
    Shin et al.~\cite{shin2020cybersecurity} & \cmarknew & Keyword-based & Text (Word2Vec) & \xmarknew \\   
    \midrule
    \textbf{\model{} (Ours)} & \cmarknew & Context-aware Classifier &  \makecell[c]{Text (BERTweet) \\ + Security Categories \\+ Temporal Information \\ + Tweet Relations (GAT)}  & \cmarknew \\
    \bottomrule
    \end{tabular}
    \label{tab:comp_baselines}
    \end{adjustbox}
\end{table*}

==> tables/classification_result_full.tex <==
\begin{table*}[h]
\footnotesize
\ra{1.5}
\caption{Tweet classification results. \textbf{Boldface} indicates the best score and \underline{underlined} indicates the second best score.}
\label{tab:classification_result_full}
\begin{adjustbox}{width=.95\textwidth, center}
\begin{tabular}{l lccc |l l ccc}
\toprule
& \textbf{Category} & \textbf{Precision} & \textbf{Recall} & \textbf{F1} &
&\textbf{Category}  & \textbf{Precision} & \textbf{Recall} & \textbf{F1} \\
\midrule
\multirow{7}{*}{\textbf{BERT}}
& Not Security related & 0.8695  & 0.9281 & 0.8978      
& \multirow{7}{*}{\textbf{RoBERTa}} 
& Not Security related & 0.8425  & 0.9432 & 0.8892 \\
& Uninformative & 0.5977 & 0.8587 & 0.7036 
& & Uninformative & 0.6187 & 0.8419  & \underline{0.7125} \\
& Data Privacy & 0.6170 & 0.7958 & 0.6940 
& & Data Privacy & 0.6158 & 0.8236 & 0.7016 \\
& Fraud/Phishing & 0.7091 & 0.8714 & \textbf{0.7812} 
& & Fraud/Phishing & 0.6843 & 0.8714 & \underline{0.7659} \\
& Ransomware/Malware & 0.8516 & 0.9122 & \textbf{0.8796} 
& & Ransomware/Malware & 0.8099 & 0.9135 & 0.8577 \\
& DDoS & 0.9367 & 0.9672 & \textbf{0.9516} 
& & DDoS & 0.9409 & 0.9493 & 0.9450 \\
& Vulnerability & 0.8862 & 0.9480 & 0.9159 
& & Vulnerability & 0.9007 & 0.9362 & 0.9179 \\
\midrule
\multirow{7}{*}{\textbf{BERTweet}} 
& Not Security related & 0.8891 & 0.9166 & \textbf{0.9025}     
& \multirow{7}{*}{\textbf{SecureBERT}} 
& Not Security related & 0.8684 & 0.9391 & \underline{0.9021} \\
& Uninformative & 0.6209 & 0.8323 & 0.7108
& & Uninformative & 0.6340 & 0.8365 & \textbf{0.7209} \\
& Data Privacy & 0.6422 & 0.8236 & \underline{0.7202}
& & Data Privacy & 0.6448 & 0.8375 & \textbf{0.7278} \\
& Fraud/Phishing & 0.6973 & 0.8486 & 0.7632
& & Fraud/Phishing & 0.6391 & 0.8657 & 0.7339 \\
& Ransomware/Malware & 0.8263 & 0.9014 & 0.8614
& & Ransomware/Malware & 0.8216 & 0.9230 & \underline{0.8691} \\
& DDoS & 0.9295 & 0.9642 &\underline{0.9459}
& & DDoS & 0.9263 & 0.9672 & 0.9461 \\
& Vulnerability & 0.9012 & 0.9424 & \underline{0.9211}
& & Vulnerability & 0.9121 & 0.9560 & \textbf{0.9334} \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table*}

==> tables/clustering_result_small.tex <==
\begin{table}[t]
\footnotesize
\ra{1.5}
\caption{Tweet Clustering Results. $\uparrow$: higher the better}
\label{tab:clustering_result}
\begin{adjustbox}{width=.75\columnwidth, center}
\begin{tabular}{lccc}
\toprule
\textbf{Model} & \textbf{AMI} ($\uparrow$)& \textbf{ARI} ($\uparrow$)& \textbf{NMI} ($\uparrow$)\\
\midrule
% Random & -0.0039 & -4.00E-05 & 0.0864 \\
TF-IDF & 0.3036 & 0.0552 & 0.5147 \\
Word2Vec & 0.0463 & 0.0060 & 0.1135 \\
\midrule
Our approach & \textbf{0.5919} & \textbf{0.3384} & \textbf{0.7344}\\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}






==> tables/data_category_detail.tex <==
\begin{table*}[ht]
\ra{2.2}
\centering
\diffnote{RC1}
\begin{mdframed}[backgroundcolor=brown!10]
\caption{Definitions and example tweets for five security categories used in our analysis. Additionally, definitions for Non-security and Uninformative categories are also included to assist the annotation process.}
\label{tab:data_category_detail}
\footnotesize
\adjustbox{width=\textwidth, center}{
\begin{tabular}{lll}
\toprule
\textbf{Category} & \textbf{Definition} & \textbf{Example Tweet} \\
\midrule
\textbf{Vulnerability} & \makecell[l]{Discussions of specific software or hardware \\ vulnerabilities, updates on patches, or newly \\ discovered exploits.} & \makecell[l]{\textit{``Cisco Releases Patches for Critical Flaws} \\ \textit{Impacting Nexus Dashboard for Data Centers''}} \\
\cmidrule{2-3}
\textbf{Ransomware/Malware} & \makecell[l]{Details about new or ongoing ransomware or malware \\ attacks, including specific incidents or general trends.} & \makecell[l]{\textit{``Symbiote: A Stealthy Linux Malware} \\ \textit{Targeting Latin American Financial Sector	''}} \\
\cmidrule{2-3}
\textbf{Data Privacy} & \makecell[l]{Issues relating to data breaches, privacy concerns, \\ or legislative changes affecting data security.} & \makecell[l]{\textit{``Kaiser Permanente Exposes Nearly 70K Medical } \\ \textit{Records in Data Breach''}} \\
\cmidrule{2-3}
\textbf{Fraud/Phishing} & \makecell[l]{Incidents or campaigns involving phishing, identity \\ theft, or other forms of cyber fraud.} & \makecell[l]{\textit{``Alert: State-Sponsored Phishing Attack Targeted } \\ \textit{Israeli Military Officials''}} \\
\cmidrule{2-3}
\textbf{DoS/DDoS} & \makecell[l]{Details about denial of service attacks, whether \\ targeted or widespread, including perpetrator and \\ mitigation details.} & \makecell[l]{\textit{``Killnet claims to have taken down the website of} \\ \textit{the (Payusatax.com) for five hours.''}} \\
\midrule
\textbf{Non-security} & \makecell[l]{Tweets not directly linked to cybersecurity issues, \\ such as job postings, promotions, general updates.} & \makecell[l]{\textit{``Join our team for a secure future in cybersecurity,} \\ \textit{apply now for our remote roles!''}} \\
\cmidrule{2-3}
\textbf{Uninformative} & \makecell[l]{Tweets that lack sufficient detail to classify into \\ a specific security category, or general statements \\ about cybersecurity without specific information.} & \makecell[l]{\textit{``Most companies will face cyber threats this year.''}} \\
\bottomrule
\end{tabular}}
\end{mdframed}
\end{table*}



==> tables/event_dataset_stat.tex <==
\begin{table}[ht]
\label{tab:clustering_dataset}
\ra{1.3}
\caption{Tweet Event Dataset}
% \vspace{}
\begin{adjustbox}{width=.5\columnwidth, center}
\begin{tabular}{ll}
\toprule
\# Events & 150 \\
\# Tweets & 1556  \\
\# Users & 764 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}


==> tables/feature_ablation.tex <==
\begin{table}[h]
\caption{Initial feature ablation study results. $\uparrow$: higher the better. $\neg$ represents the \model{} without subsequent feature}
\label{tab:feature_ablation}
\ra{1.2}
\begin{adjustbox}{width=.9\columnwidth, center}
\begin{tabular}{lccc}
\toprule
& \textbf{AMI} ($\uparrow$) & \textbf{ARI} ($\uparrow$)& \textbf{NMI} ($\uparrow$)\\
\midrule
\makecell[l]{\model \\ ($\neg$ \texttt{tweet})} & 0.5637 & 0.2712 & 0.6686 \\
\makecell[l]{\model \\ ($\neg$ \texttt{category})}  & 0.6377 & 0.3765 & 0.7462 \\
\makecell[l]{\model \\ ($\neg$ \texttt{temporal})} & 0.6459 & 0.3599 & 0.7601 \\
\midrule
\makecell[l]{\model \\ (\texttt{all})} & \textbf{0.7292} & \textbf{0.5038} & \textbf{0.8175}\\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}


==> tables/gnn_ablation.tex <==
\begin{table}[h]
\caption{GNN model ablation study results. $\uparrow$: higher the better}
\label{tab:gnn_ablation}
\ra{1.2}
\begin{adjustbox}{width=.9\columnwidth, center}
\begin{tabular}{lccc}
\toprule
& \textbf{AMI} ($\uparrow$) & \textbf{ARI} ($\uparrow$)& \textbf{NMI} ($\uparrow$)\\
\midrule
\makecell[l]{\model \\ (\texttt{GCN})} & 0.4445 & 0.1284 & 0.6507 \\
\makecell[l]{\model \\ (\texttt{GraphSAGE})}  & 0.5773 & 0.2649 & 0.7164 \\
\makecell[l]{\model \\ (\texttt{GATv2})} & \textbf{0.7292} & \textbf{0.5038} & \textbf{0.8175}\\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}


==> tables/highprofile_users.tex <==
\begin{table*}[ht]
\ra{1.2}
\caption{Examples of informative users extracted from our approach.}
\label{tab:highprofile_users}
\footnotesize
\adjustbox{width=\textwidth, center}{
\begin{tabular}{llllll}
\toprule
\textbf{User Screen Name} &\textbf{\# Followers} & \textbf{\# Following} &\textbf{User Type} & \textbf{Personal Description} \\
\midrule
TheC*** & 148,301 & 409 & - Ransomware/Malware & \makecell[l]{\textit{World's Premier Cyber Security Portal™ \#cybersecurity \#infosec} \\ \textit{\#hacking \#tech info@thecybe***}} \\

Dins***  &98,101 & 728 & \makecell[l]{- Data Privacy \\- Ransomware/Malware \\- Vulnerability} & \makecell[l]{\textit{Head of Threat \& Vulnerability Mgmt @ Henkel AG \& Co. KGaA}}\\

Peck***  &73,401 & 2 & - Fraud/Phishing & \makecell[l]{\textit{Free Chrome Extension: https://chrome.google.com/webstore/***}\\\textit{Telegram: http://t.me/***}} \\

kuri***  &44,901 & 63,901 & - Data Privacy & \makecell[l]{\textit{Co-founder @pbdlab, develop data privacy culture and collaborative} \\ \textit{measures for future data society...}} \\

\_CPR*** &19,401 & 117 & - Ransomware/Malware & \makecell[l]{\textit{Fighting cyber threats one research at a time.} \\ \textit{News from Check Po***’s (@checkpoin***) Research team.}} \\

Malw***  &8,412 & 1,722 & \makecell[l]{- Ransomware/Malware\\- DoS/DDoS} & \textit{Malware | Ransomware | Phishing | Crypto | DDoS} \\

praj*** & 1,173 & 2,487 & \makecell[l]{- Ransomware/Malware \\ - DoS/DDoS} & \makecell[l]{\textit{Assistant Editor - Global News Desk at Info***. Anything related} \\ \textit{to Cybersecurity? PLEASE DM. Tweets are personal.}}\\
\bottomrule
\end{tabular}
}
\end{table*}



==> tables/preprocess_mask.tex <==
\begin{table}[t]
\ra{1.3}
\caption{Identifiers used to replace non-linguistic element in tweets}
% \vspace{}
\label{tab:preprocess-masks}
\begin{adjustbox}{width=.8\columnwidth, center}
\begin{tabular}{ll}
\toprule
\textbf{ID Name} & \textbf{Description} \\
\midrule
\texttt{ID\_TWITTER\_URL} & Twitter URLs \\
\texttt{ID\_EMAIL\_ADDRESS} & Email addresses \\
\texttt{ID\_PHONE} & Phone numbers \\
\texttt{ID\_IP\_ADDRESS} & IPv4 and IPv6 addresses  \\
\texttt{ID\_MD5} & MD5 hash values \\
\texttt{ID\_CVE} & CVE ID \\
\texttt{ID\_NORMAL\_URL} & Refanged URLs  \\
\texttt{ID\_ONION\_URL} & Dark web onion domain URLs \\
\texttt{ID\_BTC\_ADDRESS} & Bitcoin addresses  \\
\texttt{ID\_ETH\_ADDRESS} & Ethereum addresses \\
\texttt{ID\_LTC\_ADDRESS} & Litecoin addresses \\
\texttt{ID\_LONG\_WORD} & Words with 38+ characters \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}


==> tables/text_ablation.tex <==
\begin{table}[h]
\caption{Text feature ablation study results. $\uparrow$: higher the better}
\label{tab:text_ablation}
\ra{1.5}
\begin{adjustbox}{width=.9\columnwidth, center}
\begin{tabular}{lccc}
\toprule
& \textbf{AMI} ($\uparrow$) & \textbf{ARI} ($\uparrow$)& \textbf{NMI} ($\uparrow$)\\
\midrule
\makecell[l]{\model \\ (\texttt{BERT})} & 0.6531 & 0.3659 & 0.7533 \\
\makecell[l]{\model \\ (\texttt{SecureBERT})}  & 0.6491 & 0.3896 & 0.7558 \\
\makecell[l]{\model \\ (\texttt{BERTweet})} & \textbf{0.7292} & \textbf{0.5038} & \textbf{0.8175}\\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table} 

